ExplFrame: Exploiting Page Frame Cache for Fault Analysis of Block Ciphers

Page Frame Cache (PFC) is a purely software cache, present in modern Linux based operating systems (OS), which stores the page frames that are recently being released by the processes running on a particular CPU. In this paper, we show that the page frame cache can be maliciously exploited by an adversary to steer the pages of a victim process to some pre-decided attacker-chosen locations in the memory. We practically demonstrate an end-to-end attack, ExplFrame, where an attacker having only user-level privilege is able to force a victim process's memory pages to vulnerable locations in DRAM and deterministically conduct Rowhammer to induce faults. We further show that these faults can be exploited for extracting the secret key of table-based block cipher implementations. As a case study, we perform a full-key recovery on OpenSSL AES by Rowhammer-induced single bit faults in the T-tables. We propose an improvised fault analysis technique which can exploit any Rowhammer-induced bit-flips in the AES T-tables.

==> others/ECC_attack.tex <==
\section{Fault Analysis on ECC Memory}
\label{sec:fault_on_ecc}
One critical question regarding ExplFrame and associated DRPFA attack is that whether they still hold if in-memory error correction is present. DRAMs with Error-Correcting codes (ECC) is gradually gaining popularity, and there exists several commercial instances of such hardened DRAM chips \cite{mutlu_restrospective, wiki_ecc}. It may seem that error correction can easily throttle the attacks described in this work. However, in reality, the vulnerability still holds. 

The key observation in this context is that error correction operation do incur some extra time, which eventually results in an exploitable timing channel \cite{cojocar_ecc}. Unlike the DRPFA, in this case, the attacker cannot obtain the faulty ciphertexts. Further, selective correct ciphertexts biased with the faults (just like SIFA attacks) are also unavailable. However, an attacker can still observe whether a fault induced by repeated hammering is getting corrected or not from the aforementioned timing difference. To further elaborate how this may lead to a successful attack, \emph{let us assume a scenario where the fault affects one of the T-tables of AES. This is a reasonable assumption made based on the observations from our previous experiments. Also, as we were successful in inducing Rowhammer in the T-table after a profiling phase, it is possible to pinpoint the position of the fault. Thus for simplicity, we also assume that the attacker has the knowledge of the exact fault location inside the corrupted T-table. We further assume that the attacker exactly knows which of the T-tables ($T_0$, $T_1$, $T_2$ or $T_3$) has got faulted} \footnote{We found that vulnerable locations within a page remains almost constant. Hence, if the attacker performs an initial profiling before the attack it is not difficult to infer the fault location within the table.}. Finally, we consider that the attacker can clearly identify the particular round when the error correction takes place. This is possible using the cache access based attacks namely Prime+Probe \cite{prime_probe} and Flush+Reload \cite{flush_reload} where an adversary can monitor the cache memory to determine the cache accesses corresponding to different rounds of AES execution. To ease the understanding of AES per round accesses, authors in~\cite{gullasch_cachegames, tsafrir_monopolizing} have devised methods to measure cache accesses in fine granularity. Cache accesses are utilized in this particular case to segregate between rounds of AES execution. Now, the error correction mechanism comes into play only when the faulty location is accessed. As discussed in \cite{cojocar_ecc}, the error detection and correction operations incurs a timing overhead of hundreds of thousands of clock cycles, which can be measured by the attacker. \emph{So, an attacker can easily identify the round when the faulty location gets accessed during the course of encryption.}

Referring to the structures of the T-tables and the associated AES implementation, it can be observed that each round involves $16$ table look-ups. We only focus on the cases when the error gets corrected at the very first round of AES. Rest of the cases can be discarded. \emph{Recall that an error correction takes place whenever the faulty entry in the T-table is accessed. Hence, an attacker, who can pinpoint the timing of the correction, can also deduce the input of the T-table at that time (since she has prior knowledge of which entry has got corrupted ). This input actually corresponds to one byte of the plaintext XOR-ed with one byte of the first round key. Since the plaintext is known, the key byte can be directly deduced once the T-table input is determined.} \footnote{In this context, it is worth recalling that a single round consists of total $16$ T-table look-ups. One look-up takes place for each byte of AES state. The table $T_0$ is accessed for all the bytes in the first row of the state, and similarly $T_1$, $T_2$ and $T_3$ are accessed for rows 1, 2 and 3, respectively. So, having a fault at $T_0$ in the present context helps us to extract the key-bytes corresponding to the first row elements.}

This apparently simple attack has certain critical intricacies. Most importantly, in the presence of out-of-order execution it becomes extremely difficult (if not impossible) to deduce for which byte location the error correction has taken place. In order to uniquely determine the key bytes even in this context we apply a simple trick. We begin the attack with a randomly chosen plaintext. Note that, we want the error correction to happen at the first round, and we can identify the event while it happens at the first round. The plaintext is chosen in a way so that initially there is no error correction happening. Probability of obtaining such a plaintext is fairly high (around $85$\%). Now, we vary one of the bytes of the plaintext from $0$ to $255$ keeping all other bytes constant. \emph{If faulty T-table and the location of the fault within it is fixed every time, for some value of the varying plaintext byte (let us denote the index of it by $P_i$), the error correction will take place over there (i.e. for the byte $P_i$).} Since we started with no error correction taking place in the first round, with this simple trick we can uniquely set and determine the target key byte by byte making the correction happen at the first round only for our target byte $P_0$. The entire first round key can be extracted by simply repeating this technique.

The advantage of the aforementioned trick is that it can uniquely identity the faulted byte location within a round. The round of fault, on the other hand, can be identified with the prime-and-probe as described previously. However, one should note that once the error correction takes place, the corrupted T-table becomes fault-free. In order to restart fault injection in the cipher computation, one need to perform the hammering once again. \emph{Hence, if the corruption of computation happens somewhere other than the first round, we need to restart the hammering.} A crucial question here is that \emph{how many times the hammering should be restarted before we recover one target key byte.} Below we provide a statistical estimation of this quantity.

Let us denote the event of a first round corruption as ``success'' and the event associated with the rest of the things as ``failure''. The ``failure'' event can be divided into two different sub-events -- 1) the event when no fault happens at all, and 2) the event when the fault happens at some different round. One may observe that the restart is only required for the later event. In order to estimate the number of restarts required for the extraction of a single key byte, we thus need to consider two events -- 1) the ``success'': fault happens at the first round, and 2) the ``restart'': fault happens at some different round.    

The immediate next step would be to estimate the probability of success and the probability of restart (without loss of generality we denote this event as ``failure'' from now, as we need not to bother about the event when no corruption happens). Let us denote the probability of success as $p$ and the probability of failure as $q = 1-p$. Considering the facts that only one location $t$ in a specific T-table $T_a$ gets corrupted in our experiment, and there are total $4\times10 = 40$ accesses made to $T_a$ in an entire encryption operation, the probability that no corruption (and hence no error correction) happens in an encryption is $(\frac{255}{256})^{40} = 0.855$. Consequently, the probability of at least one fault happening in an encryption is $1 -(\frac{255}{256})^{40} = 0.145$. In our experiments, the plaintext is varied only by one byte location (hence, total $256$ possible plaintexts are tested, and a ``success'' event is bound to happen within that by the properties of XOR operations). Thus, the expected number of faulty encryptions happening within these $256$ encryptions is given by $256\times 0.145 = 37.12$. 

The probability of success now can be estimated as $p = \frac{1}{37.12} = 0.026$ ($q = 1-p$). The number of restarts can now be modelled with a random variable $H$ having a truncated Geometric distribution $H \sim TGeom(n,p)$~\cite{swarup_truncated} having the probability distribution function\footnote{The main difference between the Geometric distribution with its truncated version is that the first one has an infinite support ($\{1, 2, \cdot\cdot\cdot\cdot\}$), whereas the second one has a finite support within a predefined range ($\{a+1, a+2, \cdot \cdot \cdot, b-1\}$), where $a$ and $b$ are constants defining the range.}:
\begin{equation}
    g(h) =
    \begin{cases}
     \frac{pq^{h-1}}{1-q^{d-1}}, & \text{ for } h \in \{1, 2, \cdot \cdot \cdot d-1\} \\
     0, & \text{ otherwise }
    \end{cases}
\end{equation}
Here the parameter $d$ in the distribution denote the maximum number of trials that is allowed to be performed (in our context, we know that roughly $40$ restarts (on average) are possible in total for most of the plaintext-key pairs. Hence we adopt the truncated version of Geometric distribution for modelling instead of the actual one).

We are mainly interested in estimating the mean of this distribution. With our parameter settings, the mean turns out to be roughly $16-18$. In other words, \emph{the hammering experiment (for inducing faults in the T-table) should be repeated $16-18$ times on average to extract one byte of the round key. Our experiments also support this theoretical estimation.}
%
% As a result the attacker cannot uniquely determine a key-byte. To elaborate this further let us assume that the table $T_0$ has got faulted and the attacker has the hold of this information. Now $T_0$ is accessed only for the $4$ bytes in the first row of the AES state. Evidently, the discovered T-table input can return the key for any of the 4 entries of the first row. In other words, the obtained key byte can be either the $0$th key byte, or the $4$th byte, or $8$th byte or the $12$th byte. To handle this issue we employ two simple tricks:
% \begin{enumerate}
%     \item We set the first 4 bytes of the plaintext identical. 
% \end{enumerate}

